A viable varying speed of light model in the RW metric

The Robertson-Walker (RW) metric allows us to apply general relativity to model the behavior of the Universe as a whole (i.e., cosmology). We can properly interpret various cosmological observations, like the cosmological redshift, the Hubble parameter, geometrical distances, and so on, if we identify fundamental observers with individual galaxies. That is to say that the interpretation of observations of modern cosmology relies on the RW metric. The RW model satisfies the cosmological principle in which the 3-space always remains isotropic and homogeneous. One can derive the cosmological redshift relation from this condition. We show that it is still possible for us to obtain consistent results in a specific time-varying speed-of-light model without spoiling the success of the standard model. The validity of this model needs to be determined by observations.

==> VSLRW-bib.tex <==
\begin{thebibliography}{9}

%CMB

\bibitem{Hinshaw:2013}
G.~Hinshaw \textit{et al.},  Astrophys.  J.  Suppl.  Ser.  \textbf{208},  20 (2013) doi:10.1088/0067-0049/208/2/19 [arXiv:1212.5226 [astro-ph.CO]]. 
%Nine-yearwilkinson microwave anisotropy probe (WMAP) observations: Cosmological parameter results. 

%\cite{Planck:2018nkj}
\bibitem{Planck:2018nkj}
N.~Aghanim \textit{et al.} [Planck],
%``Planck 2018 results. I. Overview and the cosmological legacy of Planck,''
Astron. Astrophys. \textbf{641}, A1 (2020)
doi:10.1051/0004-6361/201833880
[arXiv:1807.06205 [astro-ph.CO]].
%930 citations counted in INSPIRE as of 24 Jun 2022

LSS

%\cite{Guzzo:2018xbe,DES:2020sjz}
\bibitem{Guzzo:2018xbe}
L.~Guzzo, J.~Bel, D.~Bianchi, C.~Carbone, B.~R.~Granett, A.~J.~Hawken, F.~G.~Mohammad, A.~Pezzotta, S.~Rota and M.~Zennaro,
%``Measuring the Universe with galaxy redshift surveys,''
doi:10.1007/978-3-030-01629-6\_1
[arXiv:1803.10814 [astro-ph.CO]].
%1 citations counted in INSPIRE as of 24 Jun 2022

%\cite{DES:2020sjz}
\bibitem{DES:2020sjz}
R.~Cawthon \textit{et al.} [DES],
%``Dark Energy Survey Year 3 Results: Calibration of Lens Sample Redshift Distributions using Clustering Redshifts with BOSS/eBOSS,''
Mon. Not. Roy. Astron. Soc. \textbf{513}, 5517 (2022)
doi:10.1093/mnras/stac1160
[arXiv:2012.12826 [astro-ph.CO]].
%14 citations counted in INSPIRE as of 24 Jun 2022

%RW 

\bibitem{Robertson:1929}
Robertson, H. P. (1929), Proceedings of the National Academy of Sciences. {\bf 15}, (11): 822–829 (1929) doi:10.1073/pnas.15.11.822. PMC 522564. PMID 16577245.
%"On the Foundations of Relativistic Cosmology". 

\bibitem{Robertson:1933}
H.~P.~Robertson, Rev. Mod. Phys. {\bf 5}, 62 (1933) https://doi.org/10.1103/RevModPhys.5.62.
%Relativistic Cosmology

\bibitem{Walker:1935}
%On the Formal Comparison of Milne's Kinematical System with the Systems of General Relativity 
A.~G. ~Walker,  E. ~A. ~Milne,  Mon. Not. R. Astron. Soc. {\bf 95}, 263 (1935) https://doi.org/10.1093/mnras/95.3.263.

\bibitem{Walker:1937}
Walker, A. G. (1937),  Proceedings of the London Mathematical Society, Series {\bf 42}, (1): 90–127,  (1937) doi:10.1112/plms/s2-42.1.90.
%"On Milne's theory of world-structure"

%LT

\bibitem{Morin07}
D.~Morin \textit{Introduction to Classical Mechanics} (Cambridge University Press, 2007). 

%% cosmic time \cite{Weyl:1923,Islam02,Narlikar02,Hobson06,Gron07,Ryder09,CB15,Roos15,Guidry19,Ferrari21}

\bibitem{Weyl:1923}
H.~Weyl, Phys. Z. {\bf 24}, 230 (1923) (English translation: H.~Weyl, ``Republication of: On the general relativity theory'' Gen. Rel. Grav. \textbf{41}, 1661 (2009)).

\bibitem{Islam02}
J.~N.~Islam, \textit{An Introduction to Mathematical Cosmology} (Cambridge University Press, 2001).

\bibitem{Narlikar02}
J. ~V. ~Narlikar,\textit{An Introduction to Cosmology} (Cambridge University Press,  3rd Ed 2002).

\bibitem{Hobson06}
M. ~P. ~Hobson,  G.~P. ~Efstathiou,  and A. ~N. ~Lasenby, \textit{General Relativity: An Introduction for Physicists}  (Cambridge University Press,  2006).

\bibitem{Gron07} \O.~Gr\o n and S.~Hervik, \textit{Einstein's General Theory of Relativity} (Springer, 2007). 

\bibitem{Ryder09} L.~Ryder, \textit{Introduction to General Relativity} (Cambridge University Press,  2009).

\bibitem{CB15}   %\cite{Narlikar02,CB15}
Y.~ Choquet-Bruhat,  \textit{Introduction to General Relativity, Black Holes and Cosmology} (Oxford University Press,  2015). 

\bibitem{Roos15}
M.~Roos, \textit{Introduction to Cosmology} (John Wiley and Sons, 2015).

\bibitem{Guidry19}
M.~Guidry, \textit{Modern General Relativity: Black Holes, Gravitational Waves, and Cosmology} (Cambridge University Press, 2019).

\bibitem{Ferrari21}
V.~Ferrari, L.~Gualtieri, and P.~Pani, \textit{General Relativity and its Applications: Black Holes, Compact Stars and Gravitational Waves} (CRC Press, 2021).

%\cite{Lee:2020zts}
\bibitem{Lee:2020zts}
S.~Lee,
%``The minimally extended Varying Speed of Light (meVSL),''
JCAP \textbf{08}, 054 (2021)
doi:10.1088/1475-7516/2021/08/054
[arXiv:2011.09274 [astro-ph.CO]].
%5 citations counted in INSPIRE as of 16 Dec 2021

\bibitem{Weinberg:2008}
S.~Weinberg, \textit{Cosmology} (Oxford University Press, 2008). %p. 11. ISBN 978-0-19-852682-7.

 %——————— time dilation from SNe (positive) ——————————

%\cite{Leibundgut:1996qm,SupernovaSearchTeam:1997gem,Foley:2005qu,Blondin:2007ua,Blondin:2008mz}
\bibitem{Leibundgut:1996qm}
B.~Leibundgut,
%``Time dilation in the light curve of the distant type ia supernovae sn 1995k,''
Astrophys. J. Lett. \textbf{466}, L21 (1996)
doi:10.1086/310164
[arXiv:astro-ph/9605134 [astro-ph]].
%64 citations counted in INSPIRE as of 09 Dec 2022

%\cite{SupernovaSearchTeam:1997gem}
\bibitem{SupernovaSearchTeam:1997gem}
A.~G.~Riess \textit{et al.} [Supernova Search Team],
%``Time dilation from spectral feature age measurements of type ia supernovae,''
Astron. J. \textbf{114}, 722 (1997)
doi:10.1086/118506
[arXiv:astro-ph/9707260 [astro-ph]].
%60 citations counted in INSPIRE as of 09 Dec 2022


%\cite{Foley:2005qu}
\bibitem{Foley:2005qu}
R.~J.~Foley, A.~V.~Filippenko, D.~C.~Leonard, A.~G.~Riess, P.~Nugent and S.~Perlmutter,
%``A Definitive measurement of time dilation in the spectral evolution of the moderate-redshift Type Ia supernova 1997ex,''
Astrophys. J. Lett. \textbf{626}, L11-L14 (2005)
doi:10.1086/431241
[arXiv:astro-ph/0504481 [astro-ph]].
%27 citations counted in INSPIRE as of 09 Dec 2022

%\cite{Blondin:2007ua}
\bibitem{Blondin:2007ua}
S.~Blondin and J.~L.~Tonry,
%``Determining the Type, Redshift, and Age of a Supernova Spectrum,''
Astrophys. J. \textbf{666}, 1024-1047 (2007)
doi:10.1086/520494
[arXiv:0709.4488 [astro-ph]].
%321 citations counted in INSPIRE as of 09 Dec 2022

%\cite{Blondin:2008mz}
\bibitem{Blondin:2008mz}
S.~Blondin, T.~M.~Davis, K.~Krisciunas, B.~P.~Schmidt, J.~Sollerman, W.~M.~Wood-Vasey, A.~C.~Becker, P.~Challis, A.~Clocchiatti and G.~Damke, \textit{et al.}
%``Time Dilation in Type Ia Supernova Spectra at High Redshift,''
Astrophys. J. \textbf{682}, 724-736 (2008)
doi:10.1086/589568
[arXiv:0804.3595 [astro-ph]].
%37 citations counted in INSPIRE as of 09 Dec 2022




%————————— time dilation from GRBs ————————


%\cite{Norris:1993hda,Wijers:1994qf,Band:1994ee,Meszaros:1995gj,Lee:1996zu,Chang:2001fy,Crawford:2009be,Zhang:2013yna,Singh:2021jgr}
\bibitem{Norris:1993hda}
J.~P.~Norris, R.~J.~Nemiroff, J.~D.~Scargle, C.~Kouveliotou, G.~J.~Fishman, C.~A.~Meegan, W.~S.~Paciesas and J.~T.~Bonnell,
%``Detection of signature consistent with cosmological time dilation in gamma-ray bursts,''
Astrophys. J. \textbf{424}, 540 (1994)
doi:10.1086/173912
[arXiv:astro-ph/9312049 [astro-ph]].
%99 citations counted in INSPIRE as of 09 Dec 2022


%\cite{Wijers:1994qf}
\bibitem{Wijers:1994qf}
R.~A.~M.~J.~Wijers and B.~Paczynski,
%``On the nature of gamma-ray burst time dilations,''
Astrophys. J. Lett. \textbf{437}, L107 (1994)
doi:10.1086/187694
[arXiv:astro-ph/9406007 [astro-ph]].
%16 citations counted in INSPIRE as of 09 Dec 2022


%\cite{Band:1994ee}
\bibitem{Band:1994ee}
D.~Band,
%``Cosmological time dilation in gamma-ray bursts?,''
Astrophys. J. Lett. \textbf{432}, L23 (1994)
doi:10.1086/187502
[arXiv:astro-ph/9407007 [astro-ph]].
%10 citations counted in INSPIRE as of 09 Dec 2022


%\cite{Meszaros:1995gj}
\bibitem{Meszaros:1995gj}
A.~Meszaros and P.~Meszaros,
%``Cosmological evolution and luminosity function effects on number counts, redshift and time dilation of bursting sources,''
Astrophys. J. \textbf{466}, 29 (1996)
doi:10.1086/177491
[arXiv:astro-ph/9512164 [astro-ph]].
%29 citations counted in INSPIRE as of 09 Dec 2022


%\cite{Lee:1996zu}
\bibitem{Lee:1996zu}
T.~T.~Lee and V.~Petrosian,
%``Time dilation of batse gamma-ray bursts,''
Astrophys. J. \textbf{474}, 37 (1997)
doi:10.1086/303458
[arXiv:astro-ph/9607127 [astro-ph]].
%17 citations counted in INSPIRE as of 09 Dec 2022


%\cite{Chang:2001fy}
\bibitem{Chang:2001fy}
H.~Y.~Chang,
%``Fourier analysis of gamma-ray burst light curves: searching for direct signature of cosmological time dilation,''
Astrophys. J. Lett. \textbf{557}, L85 (2001)
doi:10.1086/323331
[arXiv:astro-ph/0106220 [astro-ph]].
%13 citations counted in INSPIRE as of 09 Dec 2022

%Claiming time dilation in light curves of GRBs with the anticorrelation of a timescale measure and a brightness measure has several difficulties. One difficulty is that this effect is correct only for standard candle sources with a standard duration, which we have evidence that it is not necessarily true (Kim et al. 2001; Chang & Yi 2001). A broad luminosity function and/or an intrinsic spread in the durations could smear out the signature. Another possible difficulty with this anticorrelation is that it could be mimicked by intrinsic properties of the sources (Brainerd 1994, 1997; Yi & Mao 1994; Wijers & Paczy´nski 1994). An additional complication is that an intrinsic redshift of the time profiles from higher energy bands to lower energy bands may be present (Fenimore & Bloom 1995), which would bleach the cosmological signature.

%\cite{Crawford:2009be}
\bibitem{Crawford:2009be}
D.~F.~Crawford,
%``No Evidence of Time Dilation in Gamma-Ray Burst Data,''
[arXiv:0901.4169 [astro-ph.CO]].
%8 citations counted in INSPIRE as of 09 Dec 2022

%\cite{Zhang:2013yna}
\bibitem{Zhang:2013yna}
F.~W.~Zhang, Y.~Z.~Fan, L.~Shao and D.~M.~Wei,
%``Cosmological Time Dilation in Durations of Swift Long Gamma-Ray Bursts,''
Astrophys. J. Lett. \textbf{778}, L11 (2013)
doi:10.1088/2041-8205/778/1/L11
[arXiv:1309.5612 [astro-ph.HE]].
%17 citations counted in INSPIRE as of 09 Dec 2022


%\cite{Singh:2021jgr}
\bibitem{Singh:2021jgr}
A.~Singh and S.~Desai,
%``Search for cosmological time dilation from gamma-ray bursts \textemdash{} a 2021 status update,''
JCAP \textbf{02}, no.02, 010 (2022)
doi:10.1088/1475-7516/2022/02/010
[arXiv:2108.00395 [astro-ph.HE]].
%4 citations counted in INSPIRE as of 09 Dec 2022


%———————————— cosmological time dilation QSO (negative)————

%\cite{Hawkins:2001be,Dai:2012wp}
\bibitem{Hawkins:2001be}
M.~R.~S.~Hawkins,
%``Time dilation and quasar variability,''
Astrophys. J. Lett. \textbf{553}, L97 (2001)
doi:10.1086/320683
[arXiv:astro-ph/0105073 [astro-ph]].
%17 citations counted in INSPIRE as of 09 Dec 2022

%\cite{Dai:2012wp}
\bibitem{Dai:2012wp}
D.~C.~Dai, G.~D.~Starkman, B.~Stojkovic, D.~Stojkovic and A.~Weltman,
%``Using quasars as standard clocks for measuring cosmological redshift,''
Phys. Rev. Lett. \textbf{108}, 231302 (2012)
doi:10.1103/PhysRevLett.108.231302
[arXiv:1204.5191 [astro-ph.CO]].
%7 citations counted in INSPIRE as of 09 Dec 2022





\bibitem{Lee:2212}
S.~Lee,
%``Adiabatic expansion for varying speed of light model,''
[arXiv:2212.03728 [astro-ph.CO]].
%5 citations counted in INSPIRE as of 16 Dec 2021


\end{thebibliography}


